A Louder Gravitational Wave Bang from a Fast-Expanding Universe

A strong first-order phase transition in a dark sector may produce all or part of the low-frequency gravitational wave signal recently reported by the NANOGrav Collaboration and other pulsar timing arrays. Here we point out, with a simple toy model, that even if the amplitude of the gravitational wave background from the dark phase transition is insufficient to match the NANOGrav signal, a modified expansion rate at early times may considerably enhance the gravitational wave signal. In particular, a faster-than-standard expansion rate, triggered, for instance, by the presence of one or more additional sources of energy density redshifting with higher powers of temperatures than radiation, boosts upper limits on the gravitational wave signal from first-order cosmological phase transitions, enlarging the slate of possible dark sector scenarios matching the NANOGrav signal.

==> images.tex <==
\begin{figure}
  \includegraphics[width=\columnwidth]{images/Dark_sector_phase_transition_posteriors.png}
  \caption{Recovered posterior distribution for phenomenological broken power-law parameters $f_{\ast}$ and $\Omega_{\ast}$.} 
  \label{fig:Posteriors_DSPT}
\end{figure}

\begin{figure}
  \includegraphics[width=\columnwidth]{images/DSPT_Ceffyl_Spectrum.png}
  \caption{Mean and 1$\sigma$ standard deviation contours for a set of DSPT GWB spectra with parameters drawn from the posterior distribution shown in Figure \ref{fig:Posteriors_DSPT} compared against the NANOGrav 15 year free spectrum periodograms. The value assigned to the GWB at each frequency is given in terms of a fraction of the closure density $h^2\Omega_{GW}$. } 
  \label{fig:Spectrum_DSPT}
\end{figure}

\begin{figure}
  \includegraphics[width=\columnwidth]{images/Dark_sector_phase_transition_SMBHB_posteriors.pdf}
  \caption{Same as \ref{fig:Posteriors_DSPT} but for a model containing an underlying background of astrophysical SMBHBs as well as a DSPT. The priors for the SMBHBs are informed by theoretical models.} 
  \label{fig:Posteriors_DSPT_SMBHBs}
\end{figure}

\begin{figure}
  \includegraphics[width=\columnwidth]{images/DSPT_SMBHB_Ceffyl_Spectrum.png}
  \caption{Same as \ref{fig:Spectrum_DSPT} but for the DSPT+SMBHB model. The underlying spectra for both DSPT and SMBHBs are shown in dotted and dashed lines, respectively, while their combined spectrum is shown in the solid blue line.} 
  \label{fig:Spectrum_DSPT}
\end{figure}

\begin{figure}
  \includegraphics[width=\columnwidth]{images/DSPT_only_cornerplots.png}
  \caption{Corner plots showing the number of degrees of freedom and VEV corresponding to each MCMC sample in the phenomenological model with only a DSPT and different $\xi$ values. The values of $\xi$ are 1, 2, 5, and 10 going from lightest green to darkest.} 
  \label{fig:DSPT_only_cornerplots}
\end{figure}

\begin{figure}
  \includegraphics[width=\columnwidth]{images/DSPT_SMBHB_cornerplots.png}
  \caption{Same as \ref{fig:DSPT_only_cornerplots} but for the DSPT+SMBHB model.}
  \label{fig:DSPT_only_cornerplots}
\end{figure}
